Stochastic Conditional Gradient++

In this paper, we consider the general non-oblivious stochastic optimization where the underlying stochasticity may change during the optimization procedure and depends on the point at which the function is evaluated. We develop Stochastic Frank-Wolfe++ ($\text{SFW}{++} $), an efficient variant of the conditional gradient method for minimizing a smooth non-convex function subject to a convex body constraint. We show that $\text{SFW}{++} $ converges to an $\epsilon$-first order stationary point by using $O(1/\epsilon^3)$ stochastic gradients. Once further structures are present, $\text{SFW}{++}$'s theoretical guarantees, in terms of the convergence rate and quality of its solution, improve. In particular, for minimizing a convex function, $\text{SFW}{++} $ achieves an $\epsilon$-approximate optimum while using $O(1/\epsilon^2)$ stochastic gradients. It is known that this rate is optimal in terms of stochastic gradient evaluations. Similarly, for maximizing a monotone continuous DR-submodular function, a slightly different form of $\text{SFW}{++} $, called Stochastic Continuous Greedy++ ($\text{SCG}{++} $), achieves a tight $[(1-1/e)\text{OPT} -\epsilon]$ solution while using $O(1/\epsilon^2)$ stochastic gradients. Through an information theoretic argument, we also prove that $\text{SCG}{++} $'s convergence rate is optimal. Finally, for maximizing a non-monotone continuous DR-submodular function, we can achieve a $[(1/e)\text{OPT} -\epsilon]$ solution by using $O(1/\epsilon^2)$ stochastic gradients. We should highlight that our results and our novel variance reduction technique trivially extend to the standard and easier oblivious stochastic optimization settings for (non-)covex and continuous submodular settings.

==> concave.tex <==
%!TEX root = SCG++.tex

\section{Stochastic Concave Maximization}

In this section, we focus on a another case of Problem \eqref{eqn_DR_submodular_maximization_loss} when the objective function $F$ is concave. By following the variance reduction technique, developed in the gradient approximation of \SCGPP, we introduce the \sfw method (\FWPP) for concave maximization which achieves an $\epsilon$ accurate solution in expectation after at most $\mathcal{O}(1/\epsilon^2)$ stochastic gradient computations. We study the general case of non-oblivious stochastic optimization, but, indeed, the results  also hold for the oblivious stochastic problem as a special case. 

The steps of the \FWPP are summarized in Algorithm~\ref{algo_FW++}. Unlike the update of \SCGPP, in \FWPP we restart the gradient estimation $\gB$ for the iterates that are powers of $2$. This modification is necessary to ensure that the noise of gradient approximation stays bounded by a proper constant. The rest of gradient approximation scheme is similar to that of \SCGPP. Once the gradient approximation $\gB^t$ is evaluated we find the ascent direction $\vB^t$ by solving the linear optimization program $\vB^t := \argmax_{\vB\in\CM}\{\vB^\top\gB^t\}$. Then, we compute the updated variable $\xB^{t+1}$ by performing the update $\xB^{t+1} := \xB^t + \eta_{t}\cdot(\vB^t - \xB^t)$, where $\eta_t$ is a properly chosen stepsize. 
%
%\begin{assumption}[concavity]
%	$F$ is concave.
%	\label{ass_convex}
%\end{assumption}


In the following theorem, we characterize the convergence properties of the proposed \FWPP method for solving stochastic concave maximization problems. 
For simplicity, we analyze the convergence using gradient-difference estimator \eqref{eqn_gradient_difference_estimator}.
Similar results can be obtained when using \eqref{eqn_approximate_matrix_vector_product}.


\begin{algorithm}[t]
	\caption{\sfw(\FWPP)}
	\label{algo_FW++}
	\begin{algorithmic}[1]
		\REQUIRE Number of iteration $T$, minibatch size $|\MM_0^t|$ and $|\MM_h^t|$, step size $\eta_{t} := \frac{2}{t+2}$
		\FOR{$t = 0$ \TO $T$}
		\IF{$\log_2 t \in \ZBB$}
		\STATE Sample a minibatch $\MM^t_0$ of $\zB$ with distribution $p(\zB; \xB^t)$ to compute $
			\gB^t \defi \nabla f(\xB^t; \MM_0^t)$;
		\ELSE
		\STATE Sample a minibatch $\MM_h^t$ of $\Theta$ to calculate $\tilde{\nabla}_{t}^2$ using (\ref{eqn_integral_estimator}) 
		\STATE Compute $\gB^t := \gB^{t-1} + \tilde{\nabla}_{t}^2(\xB^{t} - \xB^{t-1})$; \qquad$\diamond$ Or use \eqref{eqn_approximate_matrix_vector_product} instead.
		\ENDIF
		\STATE $\vB^t := \argmax_{\vB\in\CM}\{\vB^\top\gB^t\}$;
		\STATE $\xB^{t+1} := \xB^t + \eta_{t}\cdot(\vB^t - \xB^t)$;
		\ENDFOR
	\end{algorithmic}
\end{algorithm}
\vspace{-.3cm}


\begin{theorem}	\label{thm_convex}
Consider Problem \eqref{eqn_DR_submodular_maximization_loss} when $F$ is concave. Further, recall the \FWPP method outlined in Algorithm \ref{algo_FW++}. Let $\bar{L}^2 \defi 4B^2G^4 + 16G^4  + 4L^2 + 4B^2L^2$.
 If the conditions in Assumptions \ref{ass_upper_bound_function_value}, \ref{ass_upper_bound_stochastic_function_value}, \ref{ass_compact_domain}, \ref{ass_variance}, and \ref{ass_smooth} hold and we set \FWPP  parameters to $\eta_t = {2}/({t+2})$,  $|\MM_h^t| \!=\! 16(t\!+\!2)$ and $|\MM_0^{t}| = ({G^2(t\!+\!1)^2})/({\bar{L}^2D^2})$, then the  iterates generated by \FWPP satisfy
	\begin{equation*}
		F(\xB^*) - \EBB [F(\xB^t)]\leq \frac{28\bar{L}D^2 + (F(\xB^*) - F(\xB^0))}{t+2}.
	\end{equation*}
\end{theorem}


Theorem \ref{thm_convex} shows that after at most $\mathcal{O}(1/\epsilon)$ \FWPP reaches an $\epsilon$-approximate solution. To characterize the overall complexity, we need to take into account the number of stochastic gradient evaluations per iteration, as we do in the following corollary.
\vspace{-.1cm}
\begin{corollary}[oracle complexity for convex case]	\label{col_concave}
	Assume that the target accuracy $\epsilon$ satisfies $t\! =\! ({28LD^2\! +\! (F(\xB^*) \!-\! F(\xB^0))})/{\epsilon}  \!=\! 2^K$ for some $K \in \NBB$.
	The overall stochastic complexity is 
	\begin{equation}
		\sum_{i=0}^t |\MM_h^i| + \sum_{k=0}^{K} |\MM_0^{2^k}| \!=\! \OM\left(\frac{\bar{L}^2D^4}{\epsilon^2} \!+\! \frac{G^2D^2}{\epsilon^2} \!+\! \frac{G^2(F(\xB^*) \!- \!F(\xB^0))^2}{\bar{L}^2D^2\epsilon^2}\right).
	\end{equation}
\end{corollary}

According to Corollary \ref{col_concave}, \FWPP finds an $\epsilon$-approximate solution for stochastic concave maximization after at most computing $\mathcal{O}(1/\epsilon^2)$ stochastic gradient evaluations. %This is the best-known result in terms of overall stochastic gradient computation complexity for stochastic concave maximization (convex minimization).




==> defs.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{warning}[theorem]{Warning}
\newtheorem{question}[theorem]{Question}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}


\newdimen\pIR
\pIR= -131072sp
\newcommand\StevesR{{\rm I\kern\pIR R}}
\def\Reals#1{\StevesR^{#1}}

\def\pleq{\preccurlyeq}
\def\pgeq{\succcurlyeq}


\def\Span#1{\textbf{Span}\left(#1  \right)}
\def\bvec#1{{\mbox{\boldmath $#1$}}}


\def\prob#1#2{{\mathbb{P}}_{#1}\left[ #2 \right]}
\def\pvec#1#2{\vec{\mbox{P}}^{#1}\left[ #2 \right]}

\newcommand\symExpec{\operatorname{\mathbb{E}}\displaylimits}

\def\expec#1#2{\symExpec_{#1}  #2 }
\def\var#1{\mbox{\bf Var}\left[ #1 \right]}
\newcommand{\E}{\mbox{{\bf E}}}

\def\defeq{\stackrel{\mathrm{def}}{=}}
\def\setof#1{\left\{#1  \right\}}
\def\sizeof#1{\left|#1  \right|}




\def\floor#1{\left\lfloor #1 \right\rfloor}
\def\ceil#1{\left\lceil #1 \right\rceil}

\def\dim#1{\mathrm{dim} (#1)}
\def\sgn#1{\mathrm{sgn} (#1)}
\def\dist#1#2{\mathrm{dist} (#1, #2)}

\def\trace#1{\mathrm{Tr} \left(#1 \right)}
\def\trop{\mathrm{Tr }}


\def\union{\cup}
\def\intersect{\cap}
\def\Union{\bigcup}
\def\Intersect{\bigcap}


\def\form#1#2{\left\langle #1, #2\right\rangle}

\def\abs#1{\left|#1  \right|}


\def\norm#1{\left\| #1 \right\|}
\def\smallnorm#1{\| #1 \|}

\newcommand{\energy}[1]{\mathcal{E}\left(#1 \right)}


\def\biE{\overrightarrow{\mathrm{E}}}

\def\Reff{\mathrm{R_{eff}}}
\def\Ceff{\mathrm{C_{eff}}}

\def\calC{\mathcal{C}}
\def\calE{\mathcal{E}}
\def\calG{\mathcal{G}}
\def\calL{\mathcal{L}}
\def\calS{\mathcal{S}}



\newcommand\ddelta{\boldsymbol{\delta}}
\newcommand\Ppsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\PPsi{\boldsymbol{\mathit{\Psi}}}
\newcommand\ppsi{\boldsymbol{\mathit{\psi}}}
\newcommand\pphi{\boldsymbol{\mathit{\phi}}}
\newcommand\Llambda{\boldsymbol{\mathit{\Lambda}}}
\newcommand\PPi{\boldsymbol{\Pi}}
\def\aa{\pmb{\mathit{a}}}
\newcommand\bb{\boldsymbol{\mathit{b}}}
\newcommand\cc{\boldsymbol{\mathit{c}}}
\newcommand\dd{\boldsymbol{\mathit{d}}}
\newcommand\ee{\boldsymbol{\mathit{e}}}
\newcommand\ff{\boldsymbol{\mathit{f}}}
\renewcommand\gg{\boldsymbol{\mathit{g}}}
\newcommand\ii{\boldsymbol{\mathit{i}}}
\newcommand\jj{\boldsymbol{\mathit{j}}}
\newcommand\kk{\boldsymbol{\mathit{k}}}
\renewcommand\ll{\boldsymbol{\mathit{l}}}
\newcommand\pp{\boldsymbol{\mathit{p}}}
\newcommand\qq{\boldsymbol{\mathit{q}}}
\newcommand\bs{\boldsymbol{\mathit{s}}}
\newcommand\nn{\boldsymbol{\mathit{n}}}
\newcommand\rr{\boldsymbol{\mathit{r}}}
\renewcommand\ss{\boldsymbol{\mathit{s}}}
\def\tt{\boldsymbol{\mathit{t}}}
\newcommand\uu{\boldsymbol{\mathit{u}}}
\newcommand\vv{\boldsymbol{\mathit{v}}}
\newcommand\ww{\boldsymbol{\mathit{w}}}
\newcommand\yy{\boldsymbol{\mathit{y}}}
\newcommand\zz{\boldsymbol{\mathit{z}}}
\newcommand\xx{\boldsymbol{\mathit{x}}}

\renewcommand\AA{\boldsymbol{\mathit{A}}}
\newcommand\BB{\boldsymbol{\mathit{B}}}
\newcommand\CC{\boldsymbol{\mathit{C}}}
\newcommand\DD{\boldsymbol{\mathit{D}}}
\newcommand\GG{\boldsymbol{\mathit{G}}}
\newcommand\II{\boldsymbol{\mathit{I}}}
\newcommand\JJ{\boldsymbol{\mathit{J}}}
\newcommand\KK{\boldsymbol{\mathit{K}}}
\newcommand\NN{\boldsymbol{\mathit{N}}}
\newcommand\MM{\boldsymbol{\mathit{M}}}
\newcommand\LL{\boldsymbol{\mathit{L}}}
\newcommand\RR{\boldsymbol{\mathit{R}}}
\renewcommand\SS{\boldsymbol{\mathit{S}}}
\newcommand\UU{\boldsymbol{\mathit{U}}}
\newcommand\WW{\boldsymbol{\mathit{W}}}
\newcommand\VV{\boldsymbol{\mathit{V}}}
\newcommand\XX{\boldsymbol{\mathit{X}}}
\newcommand\mm{\boldsymbol{\mathit{m}}}

\newcommand\ppi{\boldsymbol{\pi}}
\newcommand\cchi{\boldsymbol{\chi}}
\newcommand\aalpha{\boldsymbol{\alpha}}
\newcommand\bbeta{\boldsymbol{\beta}}
\newcommand\ggamma{\boldsymbol{\gamma}}

\newcommand\xhat{\boldsymbol{\hat{\mathit{x}}}}
\newcommand\uhat{{\hat{{u}}}}
\newcommand\vhat{{\hat{{v}}}}
\newcommand\what{{\hat{{w}}}}

\newcommand\Ghat{{\widehat{{G}}}}
\newcommand\LLhat{\boldsymbol{\mathit{\widehat{L}}}}

\newcommand\thetahat{{\hat{\theta }}}



\newcommand{\sym}[1]{\mathrm{sym} (#1)}

\def\Complex#1{\mathbb{C}^{#1}}
\def\Real#1{\mathbb{R}^{#1}}

\newcommand{\imag}[1]{\mathsf{Im} (#1)}

\def\Branden{Br\"{a}nd\'{e}n}

\renewcommand{\H}{\mathcal{H}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\dan}[1]{{\bf \color{blue} Dan: #1}}
\newcommand{\nikhil}[1]{{\bf \color{green} Nikhil: #1}}
\newcommand{\adam}[1]{{\bf \color{red} Adam: #1}}

\renewcommand{\H}{\mathcal{H}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\AND}{\quad \text{and} \quad}
\newcommand{\mydet}[1]{\det\left(#1\right)}
\newcommand{\charp}[2]{\chi \left[#1 \right] \left(#2 \right)}
\newcommand{\mixed}[2]{\mu \left[#1 \right] \left(#2 \right)}



==> required.tex <==
\definecolor{myback}{RGB}{204,232,207}

\makeatletter
\newcommand{\AB}{\mathbf{A}}
\newcommand{\BB}{\mathbf{B}}
\newcommand{\CB}{\mathbf{C}}
\newcommand{\DB}{\mathbf{D}}
\newcommand{\EB}{\mathbf{E}}
\newcommand{\FB}{\mathbf{F}}
\newcommand{\GB}{\mathbf{G}}
\newcommand{\HB}{\mathbf{H}}
\newcommand{\IB}{\mathbf{I}}
\newcommand{\JB}{\mathbf{J}}
\newcommand{\KB}{\mathbf{K}}
\newcommand{\LB}{\mathbf{L}}
\newcommand{\MB}{\mathbf{M}}
\newcommand{\NB}{\mathbf{N}}
\newcommand{\OB}{\mathbf{O}}
\newcommand{\PB}{\mathbf{P}}
\newcommand{\QB}{\mathbf{Q}}
\newcommand{\RB}{\mathbf{R}}
\newcommand{\SB}{\mathbf{S}}
\newcommand{\TB}{\mathbf{T}}
\newcommand{\UB}{\mathbf{U}}
\newcommand{\VB}{\mathbf{V}}
\newcommand{\WB}{\mathbf{W}}
\newcommand{\XB}{\mathbf{X}}
\newcommand{\YB}{\mathbf{Y}}
\newcommand{\ZB}{\mathbf{Z}}
\newcommand{\zeroB}{\mathbf{0}}
\newcommand{\oneB}{\mathbf{1}}
\newcommand{\aB}{\mathbf{a}}
\newcommand{\bB}{\mathbf{b}}
\newcommand{\cB}{\mathbf{c}}
\newcommand{\dB}{\mathbf{d}}
\newcommand{\eB}{\mathbf{e}}
\newcommand{\fB}{\mathbf{f}}
\newcommand{\gB}{\mathbf{g}}
\newcommand{\hB}{\mathbf{h}}
\newcommand{\iB}{\mathbf{i}}
\newcommand{\jB}{\mathbf{j}}
\newcommand{\kB}{\mathbf{k}}
\newcommand{\lB}{\mathbf{l}}
\newcommand{\mB}{\mathbf{m}}
\newcommand{\nB}{\mathbf{n}}
\newcommand{\oB}{\mathbf{o}}
\newcommand{\pB}{\mathbf{p}}
\newcommand{\qB}{\mathbf{q}}
\newcommand{\rB}{\mathbf{r}}
\newcommand{\sB}{\mathbf{s}}
\newcommand{\tB}{\mathbf{t}}
\newcommand{\uB}{\mathbf{u}}
\newcommand{\vB}{\mathbf{v}}
\newcommand{\wB}{\mathbf{w}}
\newcommand{\xB}{\mathbf{x}}
\newcommand{\yB}{\mathbf{y}}
\newcommand{\zB}{\mathbf{z}}
\newcommand{\ZEROBB}{\mathbf{0}}
\newcommand{\ONEB}{\mathbf{1}}
\newcommand{\AMM}{\mathcal{A}}
\newcommand{\BM}{\mathcal{B}}
\newcommand{\CM}{\mathcal{C}}
\newcommand{\DM}{\mathcal{D}}
\newcommand{\EM}{\mathcal{E}}
\newcommand{\FM}{\mathcal{F}}
\newcommand{\JM}{\mathcal{J}}
\newcommand{\PM}{\mathcal{P}}
\newcommand{\TM}{\mathcal{T}}
\newcommand{\UM}{\mathcal{U}}
\newcommand{\VM}{\mathcal{V}}
\newcommand{\XM}{\mathcal{X}}
\newcommand{\YM}{\mathcal{Y}}
\newcommand{\LM}{\mathcal{L}}
\newcommand{\NM}{\mathcal{N}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\OM}{\mathcal{O}}
\newcommand{\QM}{\mathcal{Q}}
\newcommand{\HM}{\mathcal{H}}
\newcommand{\IM}{\mathcal{I}}
\newcommand{\GM}{\mathcal{G}}
\newcommand{\SM}{\mathcal{S}}
\newcommand{\RM}{\mathcal{R}}
\newcommand{\ZM}{\mathcal{Z}}
\newcommand{\ZBB}{\mathbb{Z}}
\newcommand{\RBB}{\mathbb{R}}
\newcommand{\VBB}{\mathbb{V}}
\newcommand{\EBB}{\mathbb{E}}
\newcommand{\NBB}{\mathbb{N}}
\newcommand{\varepsilonM}{\mathcal{\varepsilon}}

\newcommand{\xT}{\tilde{\mathbf{x}}}
\newcommand{\yT}{\tilde{\mathbf{y}}}
\newcommand{\zT}{\tilde{\mathbf{z}}}
\newcommand{\dHat}{\hat{\mathbf{d}}}
\newcommand{\DHat}{\hat{\mathbf{D}}}
\newcommand{\xHat}{\hat{\mathbf{x}}}
\newcommand{\alphaB}{\mbox{\boldmath$\alpha$\unboldmath}}
\newcommand{\betaB}{\mbox{\boldmath$\beta$\unboldmath}}
\newcommand{\etaB}{\mbox{\boldmath$\eta$\unboldmath}}
\newcommand{\epsilonB}{\mbox{\boldmath$\epsilon$\unboldmath}}
\newcommand{\phiB}{\mbox{\boldmath$\phi$\unboldmath}}
\newcommand{\piB}{\mbox{\boldmath$\pi$\unboldmath}}
\newcommand{\PhiB}{\mbox{\boldmath$\Phi$\unboldmath}}
\newcommand{\PsiB}{\mbox{\boldmath$\Psi$\unboldmath}}
\newcommand{\thetaB}{\mbox{\boldmath$\theta$\unboldmath}}
\newcommand{\ThetaB}{\mbox{\boldmath$\Theta$\unboldmath}}
\newcommand{\muB}{\mbox{\boldmath$\mu$\unboldmath}}
\newcommand{\SigmaB}{\mbox{\boldmath$\Sigma$\unboldmath}}
\newcommand{\GammaB}{\mbox{\boldmath$\Gamma$\unboldmath}}
\newcommand{\LambdaB}{\mbox{\boldmath$\Lambda$\unboldmath}}
\newcommand{\lambdaB}{\mbox{\boldmath$\lambda$\unboldmath}}
\newcommand{\omegaB}{\mbox{\boldmath$\omega$\unboldmath}}
\newcommand{\DeltaB}{\mbox{\boldmath$\Delta$\unboldmath}}
\newcommand{\varepsilonB}{\mbox{\boldmath$\varepsilon$\unboldmath}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\find}{\mathop{\rm find}}
\newcommand{\rank}{\mathop{\rm rank}}
\newcommand{\supp}{\mathbf{supp}}
\newcommand{\SPAN}{\mathbf{span}}
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\rk}{\mathrm{rank}}
\newcommand{\diag}{\mathsf{diag}}
\newcommand{\dg}{\mathsf{dg}}
\newcommand{\vect}{\mathsf{vec}}
\newcommand{\etal}{{\em et al.\/}\,}
\newcommand{\ie}{{\em i.e.\/}\,}
\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}
\newcommand{\prox}{\mathrm{prox}}
\newcommand{\defi}{\stackrel{\mathrm{def}}{=}}
\newcommand{\lk}{{l_k}}
\newcommand{\ik}{{i_k}}
\makeatother



\newcommand{\clr}[1]{{\color[rgb]{1,0,0} #1}}
\newcommand{\blue}[1]{{\color[rgb]{0,0,0} #1}}
\newcommand{\lightblue}[1]{{\color[rgb]{0,0,0} #1}}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{remark}{Remark}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{definition}{Definition}[section]
\newtheorem{assumption}{Assumption}
%\newtheorem{corollary}{Corollary}[section]
%\newtheorem{proposition}{Proposition}[section]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
